HyperQB: A Bounded Model Checker for Hyperproperties

We introduce the tool HyperQB 2.0, the first highly efficient push-button bounded model checker (BMC) for hyperproperties. HyperQB takes as input a model in NuSMV or Verilog and a formula expressed in the temporal logics HyperLTL or A-HLTL. The core decision procedures to implement BMC are SMT and QBF solvers, enabling verification of finite- and infinite-state programs. HyperQB offers command-line and standalone graphical, and web-based interfaces. Based on the selection of either bug-hunting or synthesis, instances of counterexamples or path witnesses are returned. The tool is entirely implemented in Rust and we report on successful and effective model checking results for a rich set of experiments on a variety of case studies with rigorous performance comparison and contrast with similar tools.

==> prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

\begin{figure}[t]
\centering
\begin{lrbox}{\nusmvbox}
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[language=NuSMV, firstnumber=1]
MODULE main
VAR
  low:  boolean; high: boolean; 
  halt: boolean; PC:   1..3;
ASSIGN
  -- Initial Conditions
  init(low)  := FALSE;
  init(high) := FALSE;
  init(halt) := FALSE;
  init(PC)   := 1;

  -- Transition Relations
  next(high) :=
    case
      (PC=1): {TRUE, FALSE};
      TRUE: high;
    esac;

\end{lstlisting}
\end{minipage}
\hfill\hspace{7mm}
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[language=NuSMV, firstnumber=19]
  next(low) :=
    case
      (PC=2 & high): TRUE;
      TRUE: low;
    esac;

  next(halt) :=
    case
      (PC=3): TRUE;
      TRUE: halt;
    esac;

  next(PC) :=
    case
      (PC<3): PC+1;
      TRUE: PC;
    esac;
\end{lstlisting}
\end{minipage}
\end{lrbox}
\scalebox{0.8}{\usebox{\nusmvbox}} 
\caption{A NuSMV model with implicit leak from \typingfont{high} to \typingfont{low}.}
\vspace{-7mm}
\label{fig:nusmv-model}
\end{figure}


\begin{wrapfigure}{r}{0.3 \textwidth}
\centering
\vspace{-15mm}
\scalebox{0.7}{
\begin{tikzpicture}[
  >=Latex,
  state/.style={
    % ellipse, draw=black!70, very thick,
    rectangle, rounded corners=5pt,
    draw=black, thin,
    % fill=black!6, 
    fill=blue!6,
    align=center,
    minimum width=20mm, minimum height=15mm,
    inner sep=2.5pt
  },
  lbl/.style={font=\scriptsize,inner sep=0pt},
  x=1mm, y=1mm
]

% --- column x-positions (left and right branch) ---
\def\xL{-15}   % left column x
\def\xR{ 15}   % right column x
\def\yTop{ 18} % s0 y
\def\dy{ -22}  % vertical gap

% s0 at top center
\node[state] (s0) at (0,\yTop) {%
  \(\neg low,~\neg high,\)\\
  \(PC = 1,\)\\
  \(\neg halt\)};

% left branch: s1 -> s2 (downwards)
\node[state] (s1) at (\xL,\yTop+\dy) {%
  \(\neg low,~high,\)\\
  \(PC = 2,\)\\
  \(\neg halt\)};
\node[state] (s2) at (\xL,\yTop+2*\dy) {%
  \(low,~high,\)\\
  \(PC=3,\)\\
  \(halt\)};

% right branch: s3 -> s4 (downwards)
\node[state] (s3) at (\xR,\yTop+\dy) {%
  \(\neg low,~\neg high,\)\\
  \(PC = 2,\)\\
  \(\neg halt\)};
\node[state] (s4) at (\xR,\yTop+2*\dy) {%
  \(\neg low,~\neg high,\)\\
  \(PC = 3,\)\\
  \(halt\)};

% labels
\node[lbl] at ($(s0.north west)+(0,2mm)$) {$s_0$};
\node[lbl] at ($(s1.west)+(-2mm,0)$) {$s_1$};
\node[lbl] at ($(s2.west)+(-2mm,0)$) {$s_2$};
\node[lbl] at ($(s3.east)+(2mm,0)$) {$s_3$};
\node[lbl] at ($(s4.east)+(2mm,0)$) {$s_4$};

% initial arrow & title
% \draw[->] ($(s0.west)+(-12mm,0)$) -- (s0.west);
% \node[lbl] at ($(s0.west)+(-18mm,0)$) {$K_{\mathrm{exp}}:$};

% transitions (downward)
\draw[->, line width=0.9pt] (s0) -- (s1);
\draw[->, line width=0.9pt] (s1) -- (s2);
\draw[->, line width=0.9pt] (s0) -- (s3);
\draw[->, line width=0.9pt] (s3) -- (s4);

\draw[red, dashed, very thick] (s1) -- (s3);
\draw[red, dashed, very thick] (s1) -- (s4);
\draw[red, dashed, very thick] (s2) -- (s4);

\end{tikzpicture}
}
\caption{The transition system of~\Cref{fig:nusmv-model}.}
\vspace{-5mm}
\label{fig:nusmv-ts}
\end{wrapfigure}

We begin by introducing the key concepts underlying our framework through illustrative examples, leaving the full formal definitions to the appendix and related references.
%
The NuSMV model in~\Cref{fig:nusmv-model} encodes a system where the low-security variable \textit{low} is updated under conditions depending on the high-security variable \textit{high}. 
%
Although no explicit flow from \textit{high} to \textit{low} exists, the model induces an implicit information leak.
% observable when branching on the value of \textit{high}. 
That is, this NuSMV model violates the \HyperLTL formula $\varphi_{\mathit{\GNI}}$ introduced in~\Cref{sec:intro}.
%
% Such leaks are not detectable by analyzing a single execution in isolation, but arise from correlations across multiple executions.

The transition system in~\Cref{fig:nusmv-ts} shows two possible executions, branching on the value of \typingfont{high}. 
%
A single trace alone cannot expose the leak, whereas hyperproperty model checking evaluates sets of traces simultaneously (e.g., comparing two traces $t_1=s_0s_1s_2$ with $t_2=s_0s_3s_4$). 
% 
Formally, given a transition system, model checking decides whether all executions, step by step through their states, collectively satisfy the desired hyperproperty.
%

Beyond synchronous reasoning, the asynchronous extension allows traces to advance at different speeds. 
%
For example, one may need to evaluate state $s_1$ on trace $t_1$ against state $s_4$ on trace $t_2$, rather than aligning them lock-step (illustrated here by following the {red dashed} alignment). 
%
Consider the LTL formula $\varphi_{eq}: \mathbf{G}(\PC_{\pi_A} = \PC_{\pi_B})$.
Under synchronous semantics (i.e., \HyperLTL), $t_1$ and $t_2$ satisfy it, since their program counters agree step by step. 
However, under asynchronous semantics (i.e., \AHLTL), the property is violated once $s_1$ on $t_1$ is compared with $s_4$ on $t_2$. 
%
This highlights the need to reason about flexible alignments, formalized through the notion of \emph{trajectories}~\cite{bcbfs21}.

Although the transition system in~\Cref{fig:nusmv-ts} is acyclic (since the NuSMV model has no loops), \HyperLTL can also be evaluated over programs with loops. 
%
In such cases, executions may be infinite, but bounded model checking leverages loop conditions to reason soundly about their behavior. 
%
Thus, even for infinite traces, one can conclude the satisfaction of global properties such as $\varphi_{eq}$ under the established \emph{loop conditions}~\cite{hsu2023efficient}.


% Model checking provides a systematic method to analyze such behaviors by exhaustively exploring the state space of the system. For hyperproperties, this entails reasoning about sets of traces rather than individual executions. In particular, logics such as HyperLTL allow quantification over multiple traces, enabling specifications of noninterference and related security properties.

% \tzuhan{Refine the text again together with what's in the Introduction.}

% \tzuhan{HyperLTL syntax. maybe 3 examples only (Kripke structure and toy examples (code, KS....}






==> tables/table_hltl.tex <==
\begin{tabular}{|c|l|c||c|c || c|c || c|c || c| c| c }
    \cline{1-11}
    & Case Study & K & Parse & Encode & HQ2.0$_{SMT}$ & AHNCE & STCE & AHCE & HQ1.0 & HQ2.0$_{QBF}$  \\ \cline{1-11}\cline{1-11}
    %%
    \multirow{17}{*}{\rotatebox{90}{TACAS 2021 cases}} 
    & BAKERY3 & $10$ & 0.02 & 0.01 & \better{0.09} & 0.72 & \bettercex{0.04} & 0.67 & \ocamlnum{6.31} & \rustnum{1.79} \\ \cline{2-10}
    & BAKERY7 & $10$ & 0.03 & 0.05 & \better{0.16} & 3.80 & \bettercex{0.06} & 1.87 & \ocamlnum{19.73} & \rustnum{3.83} \\ \cline{2-10}
    & BAKERY9 & $10$ & 0.03 & 22.17 & \better{0.17} & 6.33 & \bettercex{0.07} & 5.41 & \ocamlnum{TO} &  \\ \cline{2-10}
    & BAKERY11 & $10$ & 0.03 & 0.03 & \better{0.16} & 34.80 & \bettercex{0.07} & 33.47 & \ocamlnum{TO} &   \\ \cline{2-10}
    & SNARK1 & $18$ & 0.01 & 0.10 & \better{1.87} & 7.80 & \bettercex{0.93} & 6.38 & \ocamlnum{72.37} & \rustnum{2.01} & * \\ \cline{2-10}
    % & SNARK2 & ? & ? & ? & ? & ? & ? & ?  & ? \\ \cline{2-10}
    & NI$_{Correct}$ & $50$ & 0.03 & 0.11 & 1.43 & \better{0.62} & - & - & \ocamlnum{1.40} & \rustnum{1.53} \\ \cline{2-10}
    & NI$_{Inorrect}$ & $50$ & 0.03 & 0.11 & \better{1.38} & 2.59 & 7.20 & \bettercex{1.91} & \ocamlnum{5.24} &\rustnum{1.52} \\ \cline{2-10}
    & NRP$_{Correct}$ & $15$ & 0.02 & 0.01 & \better{0.16} & 0.70 & - & - & \ocamlnum{0.96} & \rustnum{0.85} \\ \cline{2-10}
    & NRP$_{Incorrect}$ & $15$ & 0.01 & 0.01 & \better{0.13} & 1.21 & - & - & \ocamlnum{1.05} & \rustnum{0.83} \\ \cline{2-10}
    & Robust $10^2$ & $20$ & 0.03 & 0.04 & \forq{\better{0.38}} & \forq{5.11} & - & -& \ocamlnum{3.01} & \rustnum{1.51} \\ \cline{2-10}
    & Robust $20^2$ & $40$ & 0.05 & 0.11 & \forq{\better{4.05}} & \forq{22.47} & - & - & \ocamlnum{10.05} & \rustnum{5.66} & * \\ \cline{2-10}
    & Robust $40^2$ & $80$ & 0.08 & 0.97 & \forq{\better{9.13}} & \forq{209.87} & - & - & \ocamlnum{110.60} & \rustnum{19.67} &  * \\ \cline{2-10}
    & Robust $60^2$ & $120$ & 0.13 & 6.78 & \better{1233.39} & \forq{TO} & - & - & \ocamlnum{478.42} & \rustnum{129.88} & \# \\ \cline{2-10}
    & SP $10^2$ & $20$ & 0.03 & 0.08 & \better{0.67} & 5.23 & - & - & \ocamlnum{6.53} & \rustnum{2.01}  \\ \cline{2-10}
    & SP $20^2$ & $40$ & 0.05 & 0.96 & {32.75} & \better{13.61} & - & - & \ocamlnum{110.48} & \rustnum{TO}  \\ \cline{2-10}
    & SP $40^2$ & $80$ & 0.05 & 26.96 & \forq{TO} & \better{85.56} & - & -& \ocamlnum{TO} & \rustnum{TO} \\ \cline{2-10}
    & SP $60^2$ & $120$ & 0.08 & 3.56 & \forq{TO} & \better{41.24} & - & - & \ocamlnum{TO} & \rustnum{TO}  \\ \cline{2-10}
    & Mutation & $10$ & 0.02 & 0.01 & \better{0.05} & 0.52 & - & -& \ocamlnum{0.83} & \rustnum{0.85} \\ \cline{1-10}\cline{1-10}

    %%
    \multirow{16}{*}{\rotatebox{90}{HyperQB 1.0 arXiv cases}} 
    & Co-termination & $10$ & 0.01 & 0.00 & \better{0.01} & 0.30 & - & - & \ocamlnum{1.65} & \rustnum{0.90} \\ \cline{2-10}
    & Deniability & $10$ & 0.02 & 0.01 & \better{0.15} & \forq{11.56} & - & - & \ocamlnum{105.23} & \rustnum{17.78}  \\ \cline{2-10}
    & Buffer$_{OD^{classic}}$ & $10$ & 0.01 & 0.01 & \better{0.04} & 0.43 & \bettercex{0.04} & 0.85 & \ocamlnum{2.70} & \rustnum{0.88}  \\ \cline{2-10}
    & Buffer$_{OD^{intr}}$ & $10$ & 0.01 & 0.01 & \better{0.04} & 0.68 & - & - & \ocamlnum{2.63} & \rustnum{0.82} \\ \cline{2-10}
    & Buffer$_{GMNI^{intr}}$ & $10$ & 0.01 & 0.01 & \better{0.09} & 2.69 & - & - & \ocamlnum{1.42} & \rustnum{0.81} \\ \cline{2-10}
    & Buffer$_{OD^{classic}}$ & $10$ & 0.02 & 0.00 & \better{0.03} & 0.56 & \bettercex{0.04} & 9.11 & \ocamlnum{1.24} & \rustnum{0.82}  \\ \cline{2-10}
    & Nodet$_{TINI}$ & $10$ & 0.01 & 0.00 & \better{0.09} & \forq{1.85} & - & -  & \ocamlnum{2.31} & \rustnum{0.77} \\ \cline{2-10}
    & Nodet$_{TSNI}$ & $10$ & 0.02 & 0.01 & \better{0.08} & \forq{1.83} & - & - & \ocamlnum{2.35} & \rustnum{0.78}  \\ \cline{2-10}
    & K-Safety & $10$ & 0.01 & 0.02 & \doublecheck{6.89} & \better{0.49} & - & - & \ocamlnum{2.84} &  \\ \cline{2-10}
    & MapSynth 1 & $10$ & 0.03 & 0.01 & \better{0.07} & 0.50 & - & - & \ocamlnum{0.79}  &  \\ \cline{2-10}
    & MapSynth 2 & $10$ & 0.02 & 0.00 & \better{30.27} & \forq{TO} & - & - & \ocamlnum{9.49} & & *  \\ \cline{2-10}
    & Team LTL 1 & $10$ & 0.01 & 0.01 & 1.39 & \better{0.36} & - & - & \ocamlnum{1.58} & \rustnum{0.92} \\ \cline{2-10}
    & Team LTL 2 & $10$ & 0.01 & 0.01 & 2.42 & \better{0.89} & - & - & \ocamlnum{60.08} & \rustnum{0.93}  \\ \cline{2-10}
    & NDET v1 & $10$ & 0.01 & 0.00 & \better{0.03} & 0.31 & \bettercex{0.03} & 0.34 & \ocamlnum{0.69} & \rustnum{0.76} \\ \cline{2-10}
    & NDET v2 & $10$ & 0.01 & 0.00 & \better{0.04} & \forq{0.35} & \bettercex{0.03} & \forq{TO}  & \ocamlnum{0.73} & \rustnum{0.81} & * \\ \cline{2-10}
    & NDET v3 & $10$ & 0.01 & 0.00 & \better{0.04} & \forq{68.99} & \bettercex{0.03} & \forq{TO} & \ocamlnum{0.76} & \rustnum{0.84} & \#   \\ \cline{1-10}\cline{1-10}
    %%
    \multirow{13}{*}{\rotatebox{90}{HyperQB 2.0 new cases}} 
    & Bank v1 & $10$ & 0.02 & 0.01 & \better{0.10} & 0.53 & \bettercex{0.04} & 11.48 & \ocamlnum{51.45} & \rustnum{0.87}  \\ \cline{2-10} 
    & Bank v2 & $10$ & 0.02 & 0.01 & \better{0.06} & 0.32 & \bettercex{0.05} & 0.68 & \ocamlnum{2.68} & \rustnum{0.83}  \\ \cline{2-10} 
    & Bank v3 & $10$ & 0.02 & 0.01 & \better{0.07} & 0.33 & \bettercex{0.04} & 0.74 & \ocamlnum{2.16} & \rustnum{0.82} \\ \cline{2-10} 
    & Constructor & $10$ & 0.02 & 0.01 & \better{0.08} & 0.58 & \bettercex{0.08} & 0.42 & \ocamlnum{1.77} & \rustnum{0.89}   \\ \cline{2-10}
    & Bidding v1 & $10$ & 0.01 & 0.01 & \better{0.01} & 0.28 & - & - & \ocamlnum{0.73} & \rustnum{0.95} \\ \cline{2-10}
    & Bidding v2 & $10$ & 0.01 & 0.01 & \better{0.01} & 0.29 & - & - & \ocamlnum{0.86} & \rustnum{0.89} \\ \cline{2-10}
    & Bidding v3 & $10$ & 0.02 & 0.01 & \better{0.02} & 0.68 & - & - & \ocamlnum{30.61} & \rustnum{1.07} \\ \cline{2-10}
    & Bidding v4 & $10$ & 0.01 & 0.01 & \better{0.05} & 0.32 & \bettercex{0.03} & 2.81 & \ocamlnum{1.89} & \rustnum{0.95}   \\ \cline{2-10}
    & IQueue & $10$ & 0.03 & 0.06 & \better{0.73} & \forq{TO} & \bettercex{0.59} & \forq{TO} & \ocamlnum{68.06} & & *  \\ \cline{2-10}
    & Keypad & $10$ & 0.01 & 0.01 & \better{0.02} & 14.57 & - & - &  \ocamlnum{1.48} & & *  \\ \cline{2-10}
    & Simple queue & $10$ & 0.02 & 0.03 & \better{0.02} & 0.27 & \bettercex{0.02} & 0.22  & \ocamlnum{0.75} & \\ \cline{2-10} 
    & EMM ABA & $10$ & 0.03 & 0.02 & \better{0.12} & \forq{72.52} & 0.07 & \forq{TO} & \ocamlnum{88.14} &  & * \\ \cline{2-10} 
    & Lazy List & $13$ & 0.03 & 0.05 & \better{0.40} & \forq{TO} & \bettercex{0.20} & \forq{TO} & \ocamlnum{TO} & \rustnum{1.23} & \# \\ \cline{1-10}\cline{1-10}
\end{tabular}



